Certified Compilation in the TELEPERM XS Nuclear Safety I&C Platform

The large safety instrumentation & control (I&C) systems in civil nuclear power plants (NPPs) are mainly safe-shutdown systems (reactor protection) or limitation and control systems. Framatome's established TELEPERM XS (TXS Core) product family is a digital I&C system platform to cover all these applications. We illustrate the role of verification in the different stages of the software production toolchain, focus on the formal compilation process, and discuss the contribution of the CompCert certified compiler to the safety case of the product. Scrutinizing the object code produced by this compiler has exhibited suboptimal run-time performance in a certain simple but recurring generated code pattern. We explain how formal methods allow us to address this issue in the compiler while simultaneously reducing its trusted computing base (TCB), thereby strengthening the safety case rather than merely preserving it.

==> eptcsdata.tex <==
\providecommand{\firstpage}{92}
\providecommand{\publicationstatus}{Mircea Marin, Adrian Cr\u{a}ciun (Eds.): FROM 2026\\
EPTCS 452, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.452.7}{10.4204/EPTCS.452.7}}
\pdfoutput=1

